A tensor network formulation of Lattice Gauge Theories based only on symmetric tensors

The Lattice Gauge Theory Hilbert space is divided into gauge-invariant sectors selected by the background charges. Such a projector can be directly embedded in a tensor network ansatz for gauge-invariant states as originally discussed in [Phys. Rev. B 83, 115127 (2011)] and in [Phys. Rev. X 4, 041024 (2014)] in the context of PEPS. The original ansatz is based on sparse tensors, though parts of them are not explicitly symmetric, and thus their actual implementation in numerical simulations has been hindered by the complexity of developing ad hoc libraries. Here we provide a new PEPS tensor network formulation of gauge-invariant theories purely based on symmetric elementary tensors. The new formulation can be implemented in numerical simulation using available state-of-the-art tensor network libraries but also holds interest from a purely theoretical perspective since it requires embedding the original gauge theory with gauge symmetry G into an enlarged globally symmetric theory with symmetry GxG. By revisiting the original ansatz in the modern landscape of i) duality transformations between gauge and spin systems, ii) finite depth quantum circuits followed by measurements that allow generating topologically ordered states, and iii) Clifford enhanced tensor networks, we show that such a new formulation provides a novel duality transformation between lattice gauge theories and specific sectors of globally invariant systems.

==> editions/onetimestep.tex <==
\ensuremath{
\begin{matrix}
    \includegraphics[scale=0.8]{images/onetimestep.pdf}
\end{matrix}
}

==> editions/opR.tex <==
\ensuremath{
\begin{matrix}
    \includegraphics[scale=1.1]{images/MPO.pdf}
\end{matrix}
% EDIT 1
\def \myx {7pt}
\def \myy {0pt}
\hspace{-\myx}
\raisebox{\myy}{
$R$
}
\hspace{\myx}
% CHECK CURSOR
\hspace{-5pt}
}

==> editions/rotatedten_zn_v2.tex <==
\ensuremath{
% IMAGE
\begin{matrix}
    \includegraphics[scale=1.7]{images/example_gral4leg.pdf}
\end{matrix}
% FIRST LEG: Ra
\def \myx {93pt}
\def \myy {-3pt}
\hspace{-\myx}
\raisebox{\myy}{$
R_a^{[1]}
$}
\hspace{\myx}
% FIRST LEG: dot
\def \myx {93pt}
\def \myy {-11.5pt}
\hspace{-\myx}
\raisebox{\myy}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \filldraw (0,0) circle (1.5pt);
\end{tikzpicture}
$}
\hspace{\myx}
% FIRST LEG: arrow 1
\def \myx {97pt}
\def \myy {-8pt}
\def \myangle {42}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% FIRST LEG: arrow 2
\def \myx {119pt}
\def \myy {-17pt}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% k LEG: Ra
\def \myx {70pt}
\def \myy {-20pt}
\def \dx {-7pt}
\hspace{-\myx}
\hspace{\dx}
\raisebox{\myy}{$
R_a^{[k]}
$}
\hspace{\myx}
\hspace{-\dx}
% k LEG: dot
\def \myx {102.5pt}
\def \myy {-16pt}
\hspace{-\myx}
\raisebox{\myy}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \filldraw (0,0) circle (1.5pt);
\end{tikzpicture}
$}
\hspace{\myx}
% k LEG: arrow 1
\def \myx {110pt}
\def \myy {-12.5pt}
\def \myangle {70}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% k LEG: arrow 2
\def \myx {124.7pt}
\def \myy {-21.7pt}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% k+1 LEG: Ra
\def \myx {100pt}
\def \myy {-7pt}
\hspace{-\myx}
\raisebox{\myy}{$
(R_a^{[k+1]})^\dagger
$}
\hspace{\myx}
% k+1 LEG: dot
\def \myx {141pt}
\def \myy {4.7pt}
\hspace{-\myx}
\raisebox{\myy}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \filldraw (0,0) circle (1.5pt);
\end{tikzpicture}
$}
\hspace{\myx}
% k+1 LEG: arrow 1
\def \myx {155.5pt}
\def \myy {2.4pt}
\def \myangle {11}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% k+1 LEG: arrow 2
\def \myx {151pt}
\def \myy {4.8pt}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% J LEG: Ra
\def \myx {240pt}
\def \myy {18pt}
\hspace{-\myx}
\raisebox{\myy}{$
(R_a^{[J]})^\dagger
$}
\hspace{\myx}
% J LEG: dot
\def \myx {233pt}
\def \myy {19.5pt}
\hspace{-\myx}
\raisebox{\myy}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \filldraw (0,0) circle (1.5pt);
\end{tikzpicture}
$}
\hspace{\myx}
% J LEG: arrow 1
\def \myx {241pt}
\def \myy {23pt}
\def \myangle {76}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% J LEG: arrow 2
\def \myx {254.7pt}
\def \myy {13.5pt}
\hspace{-\myx}
\raisebox{\myy}{
\rotatebox[origin=c]{\myangle}{$
\begin{tikzpicture}[line width=1.5pt, color=gray!165]
    \draw [-{Classical TikZ Rightarrow[length=3.5pt]}](0,0) -- (0.05,0);
\end{tikzpicture}
$}}
\hspace{\myx}
% dots 1
\def \myx {245pt}
\def \myy {18pt}
\hspace{-\myx}
\raisebox{\myy}{$\dots$}
\hspace{\myx}
% dots 2
\def \myx {280pt}
\def \myy {-15pt}
\hspace{-\myx}
\raisebox{\myy}{$\dots$}
\hspace{\myx}
% CHECK CURSOR
\hspace{-200pt}
}

==> sections/I_aknowledgments.tex <==


\begin{acknowledgments}
    I would like to thank Luca Tagliacozzo for his dedication and his mentoring and Jan von Delft for the opportunity to work in his group.
\end{acknowledgments}

==> sections/sections_v1/I_aknowledgments.tex <==


\begin{acknowledgments}
    I would like to thank Luca Tagliacozzo for his dedication and his mentoring and Jan von Delft for the opportunity to work in his group.
\end{acknowledgments}

==> sections/sections_v2/I_aknowledgments.tex <==


\begin{acknowledgments}
    I would like to thank Luca Tagliacozzo for his dedication and his mentoring and Jan von Delft for the opportunity to work in his group.
\end{acknowledgments}

==> sections/sections_v2/I_aknowledgments_luca.tex <==


\begin{acknowledgments}
 This work summarizes some of the results of the master thesis of MC. The thesis started from some preliminary discussions that we had with Natalia Chepiga, in order to uniformize the approach they use in contrained DMRG \cite{chepiga2019} with the approach that we use in gauge invariant tensor networks \cite{tagliacozzo2014}. Such discussions gave rise to a similar ansatz to the one described in \cite{silvi2014}, where the Hilbert space on the link is doubled, and one then absorb each copy of the link onto the closest vertex and then imposing an independent $U(1)$ symmetry constraint on every link of the lattice. The one dimensional formulation is particularly easy  and lead to several unpublished numerical simulations performed together with Umberto Borla using TenPy. We thank both Umberto and Natalia for discussions and work on those related formulations hoping we will eventually write a paper summarizing our results. MC thesis was meant to generalize such an approach to 2D. However we soon realized that in 2D such an approach would require to work with prohibitively large PEPS tensors, since in two dimensions, on the square lattice, each vertex would need to absorb $4$ copies of the link Hilbert space.

 While such an approach has been succesfully pursued by the group of Montangero using Tree Tensor networks, we have realized that the PEPS ansatz could still be mantained as simple as the original gauge invariant ansatz in \cite{tagliacozzo2014} by doubling the symmetries on the links rather than doubling the number of constituents on them  during the intial stages of MC's thesis and given the theoretical relevance of such an observation we have decided to publish these results separately.

 MC was hosted by Jan Von Delft during his thesis and we would like to thank him and his group for the support and the discussions on this topic we had during the thesis.

LT acknowledge support from the Proyecto Sinérgico CAM Y2020/TCS-6545 NanoQuCo-CM,
the CSIC Research Platform on Quantum Technologies PTI-001, and from the Grant TED2021-130552B-C22 funded by MCIN/AEI/10.13039/501100011033 and by the ``European Union NextGenerationEU/PRTR'',
and Grant PID2021-127968NB-I00 funded by MCIN/AEI/10.13039/501100011033

\end{acknowledgments}

